Participation Cost Estimation: Private Versus Non-Private Study

In our study, we seek to learn the real-time crowd levels at popular points of interests based on users continually sharing their location data. We evaluate the benefits of users sharing their location data privately and non-privately, and show that suitable privacy-preserving mechanisms provide incentives for user participation in a private study as compared to a non-private study.

==> architecture.tex <==
\section{Architecture}

The existing system consists of three components: analysts, data owners, and the aggregator.

\subsection{Analysts}

An analyst formulates queries, distributes the queries to data owners via the aggregator, and receives the query results from the aggregator. Multiple analysts can operate in the system simultaneously. Each query is signed by the analyst. Each analyst is expected to be reputable. Examples of an analyst may be the Los Angeles Depart of Transportation, Centers for Disease Control, or National Institutes of Health.


\subsection{Data Owners}

A data owner is a user device under the user's control.  It stores the continuously-generated personal user data locally.  Each data owner requests queries from specific analysts, answers these queries over the data owners's local data, and responds either by transmitting the non-privatized answer or by replying with the randomized response mechanism .

\subsection{Aggregator}

The aggregator mediates between the analysts and data owners. If the proxy is not used in the design, the analysts need to connect to numerous clients for collecting data. Also, the clients will be unaware of what analysts to trust. Hence a distributed proxy is used for this purpose. Using the query answers provided by the individuals who participated in the study, the system aims to calculate the congestion at the several locations in and around UCLA.

\subsection{Design}

The important phases involved in the design of the system (which is an iOS app) are as follows:
Messages are read from the proxy at regular intervals for queries from the analysts.
The queries are stored in a queue for threads to read one query at a time from the queue. This also involves a thread, which will delete the data from the queue based on the QueryEndTime of each query. 
Threads run in parallel to generate the required sensor data and combine them into the answer object and send to the Data Transfer module 
The data transfer module then pushes the encrypted and randomized responses along with the key to the objects, to the proxy for each epoch. The proxy then forwards these responses to the analysts.
Thus, continuous real time collection of the data takes place in the system through the responses collected during each epoch. The workflow of the events in the system are shown in Figure 1 which is taken from [4]
